Efficient Bilevel Source Mask Optimization

Resolution Enhancement Techniques (RETs) are critical to meet the demands of advanced technology nodes. Among RETs, Source Mask Optimization (SMO) is pivotal, concurrently optimizing both the source and the mask to expand the process window. Traditional SMO methods, however, are limited by sequential and alternating optimizations, leading to extended runtimes without performance guarantees. This paper introduces a unified SMO framework utilizing the accelerated Abbe forward imaging to enhance precision and efficiency. Further, we propose the innovative \texttt{BiSMO} framework, which reformulates SMO through a bilevel optimization approach, and present three gradient-based methods to tackle the challenges of bilevel SMO. Our experimental results demonstrate that \texttt{BiSMO} achieves a remarkable 40\% reduction in error metrics and 8$\times$ increase in runtime efficiency, signifying a major leap forward in SMO.

==> doc/res/epe.tex <==
\begin{table}[!htp]\centering
  \caption{EPE comparison.}\label{tab:epe}
  \resizebox{.96\linewidth}{!}{
  \begin{tabular}{|c|ccc|cc|ccc|}\hline
      \multirow{2}{*}{Bench} &\multicolumn{3}{c|}{MO} &\multicolumn{2}{c|}{\texttt{AM-SMO}} & &\texttt{BiSMO} & \\\cline{2-9} %\cmidrule{2-9}
  &{\small \makecell{NILT\\\cite{OPC-ICCAD2020-NeuralILT}}} &{\makecell{\small DAC\\23\cite{multiilt2023sun}}} &\makecell{\small Abbe\\-MO} &\makecell{\small A$\sim$H$^\star$\\\cite{ding2020gradient}} &\makecell{\small A$\sim$A$\dagger$\\\cite{sampleICC2022sun}} &\texttt{FD} &\texttt{CG} & \texttt{NMN} \\\hline \hline
  ICCAD &7.5 &2.5 &1.9 &2.4 &1.7 &1.3 &1.3 &1.3 \\
  ICCAD-L &10.7 &3.5 &2.6 &3.3 &2.1 &1.6 &1.5 &1.5 \\
  ISPD19 &12 &4.8 &3.8 &4.3 &3.3 &2.7 &2.5 &2.4 \\\hline
  Average &10.1 &3.6 &2.8 &3.3 &2.4 &1.9 &1.8 &1.7 \\
  Ratio &5.8 &2.1 &1.6 &1.9 &1.4 &1.1 &1.0 &1.0 \\
  \hline
  \multicolumn{9}{l}{\small{A$\sim$H$^\star$: Abbe-Hopkins; A$\sim$A$\dagger$: Abbe-Abbe.}} \\
  \end{tabular}
  }
\end{table}


==> doc/res/epe_small.tex <==
\begin{table}[!htp]\centering
  \caption{EPE comparison.}\label{tab:epe}
  \setlength{\tabcolsep}{3pt}
  \begin{tabular}{c|ccc|c|c}\toprule
  \multirow{2}{*}{Bench} &\multicolumn{3}{c|}{MO} &\texttt{AM-SMO} &\texttt{BiSMO} \\%\cmidrule{2-6}
  &{\small \makecell{NILT\\\cite{OPC-ICCAD2020-NeuralILT}}} &{\makecell{DAC\\23\cite{multiilt2023sun}}} &Abbe-MO &{\small Abbe-Abbe\cite{sampleICC2022sun}} &\texttt{NMN} \\\midrule
  ICCAD &7.5 &2.5 &1.3 &1.1 &0.9 \\
  ICCAD-L &10.7 &3.5 &1.5 &1.4 &1.2 \\
  ISPD &12 &4.8 &2.7 &2.5 &1.9 \\\midrule
  Average &10.1 &3.6 &1.8 &1.7 &\textbf{1.3} \\
  Ratio &7.55 &2.7 &1.375 &1.25&\textbf{1} \\
  \bottomrule
  \end{tabular}
\end{table}

==> doc/res/ibm.tex <==
\begin{table*}[!htp]\centering
  \caption{Generated by Spread-LaTeX}\label{tab:ibm_all}
  \setlength{\tabcolsep}{3pt}
	\renewcommand{\arraystretch}{1}
  \begin{tabular}{c|cc|cc|cc|cc|cc|cc|cc}\toprule
  {Bench} &\multicolumn{4}{c|}{MO} &\multicolumn{4}{c|}{\texttt{AM-SMO}} &\multicolumn{6}{c}{\texttt{BiSMO} (Ours)} \\\cmidrule(lr){1-1} \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-15}
  \multirow{2}{*}{ID}&\multicolumn{2}{c|}{\small MultiILT[DAC23]} &\multicolumn{2}{c|}{Abbe-MO (Ours)} &\multicolumn{2}{c|}{Abbe-Hopkins} &\multicolumn{2}{c|}{Abbe-Abbe [12,13]} &\multicolumn{2}{c|}{\texttt{BiSMO-FD}} &\multicolumn{2}{c|}{\texttt{BiSMO-CG}} &\multicolumn{2}{c}{\texttt{BiSMO-NMN}} \\
  &L2 &PVB &L2 &PVB &L2 &PVB &L2 &PVB &L2 &PVB &L2 &PVB &L2 &PVB \\\midrule%\cmidrule(lr){1-1} \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-15}
  case1 &39303 &46077 &23167 &27525 &38187 &43228 &23444 &23675 &19571 &19777 &18118 &19091 &17918 &18589 \\
  case2 &28986 &37627 &18542 &24030 &27481 &35334 &16174 &20678 &14756 &17754 &14818 &16058 &14045 &16640 \\
  case3 &66151 &68021 &29203 &28290 &64950 &65089 &27861 &24759 &25784 &21604 &28448 &19522 &25508 &19980 \\
  case4 &15890 &23511 &9916 &15148 &14316 &20525 &8090 &12776 &6734 &10540 &6333 &9404 &6330 &8862 \\
  case5 &29138 &49987 &17986 &28574 &28047 &46447 &16623 &24923 &14945 &22315 &15314 &19746 &14846 &19430 \\
  case6 &30558 &44503 &18171 &28374 &28887 &41543 &17500 &24668 &15365 &22397 &13906 &19425 &13458 &18923 \\
  case7 &15765 &37009 &11776 &22439 &14791 &35213 &9980 &19684 &8240 &16842 &8672 &14634 &8161 &13362 \\
  case8 &13943 &21503 &11144 &16246 &12961 &18281 &9696 &13842 &8301 &11541 &7702 &9877 &7568 &9384 \\
  case9 &36397 &55600 &20075 &32024 &35283 &52001 &19956 &27679 &17526 &25127 &15923 &24339 &15971 &23067 \\
  case10 &7492 &16604 &7712 &14316 &8043 &15040 &7268 &12756 &7053 &10824 &6796 &10648 &6788 &10156 \\\midrule
  Avg. &28362.3 &40044.2 &16769.2 &23696.6 &27294.6 &37270.1 &15659.2 &20544 &13827.5 &17872.1 &13603 &16274.4 &\textbf{13059.3} &\textbf{15839.3} \\
  Ratio &2.17 &2.53 &1.28 &1.50 &2.09 &2.35 &1.20 &1.30 &1.06 &1.13 &1.04 &1.03 &\textbf{1.00} &\textbf{1.00} \\
  \bottomrule
  \end{tabular}
  \end{table*}
